PlaneMatch: Patch Coplanarity Prediction for Robust RGB-D Reconstruction

We introduce a novel RGB-D patch descriptor designed for detecting coplanar surfaces in SLAM reconstruction. The core of our method is a deep convolutional neural net that takes in RGB, depth, and normal information of a planar patch in an image and outputs a descriptor that can be used to find coplanar patches from other images.We train the network on 10 million triplets of coplanar and non-coplanar patches, and evaluate on a new coplanarity benchmark created from commodity RGB-D scans. Experiments show that our learned descriptor outperforms alternatives extended for this new task by a significant margin. In addition, we demonstrate the benefits of coplanarity matching in a robust RGBD reconstruction formulation.We find that coplanarity constraints detected with our method are sufficient to get reconstruction results comparable to state-of-the-art frameworks on most scenes, but outperform other methods on standard benchmarks when combined with a simple keypoint method.

==> intro_lr.tex <==
\begin{figure}[b!] \centering
    \begin{overpic}[width=0.999\linewidth]{intro_lr_fig.pdf}\small
    \put(15,-2){Coplanarity + Key-point}
    \put(70,-2){Key-point only}
    \end{overpic}
    \caption{Benefit of long-range coplanarity in aligning large-scale sequence. The scans for the long flat wall and floor are mis-aligned by key-points only (right) while well-registered with coplanarity constraints added (left).}
    \label{fig:introlr}
\end{figure} 
